A Novel Fast Exact Subproblem Solver for Stochastic Quasi-Newton Cubic Regularized Optimization

In this work we describe an Adaptive Regularization using Cubics (ARC) method for large-scale nonconvex unconstrained optimization using Limited-memory Quasi-Newton (LQN) matrices. ARC methods are a relatively new family of optimization strategies that utilize a cubic-regularization (CR) term in place of trust-regions and line-searches. LQN methods offer a large-scale alternative to using explicit second-order information by taking identical inputs to those used by popular first-order methods such as stochastic gradient descent (SGD). Solving the CR subproblem exactly requires Newton's method, yet using properties of the internal structure of LQN matrices, we are able to find exact solutions to the CR subproblem in a matrix-free manner, providing large speedups and scaling into modern size requirements. Additionally, we expand upon previous ARC work and explicitly incorporate first-order updates into our algorithm. We provide experimental results when the SR1 update is used, which show substantial speed-ups and competitive performance compared to Adam and other second order optimizers on deep neural networks (DNNs). We find that our new approach, ARCLQN, compares to modern optimizers with minimal tuning, a common pain-point for second order methods.

==> Convergence.tex <==
\section{Convergence analysis}  \label{sec:convergence} 

\begin{comment}
\begin{assumption} \label{as:flowerbound}
The function $f(x)$ is bounded below by a scalar $L_f$
\end{assumption}

\begin{assumption} \label{as:gLipschitz}
$g(x)$ are L-Lipschitz continuous for all $x$
\end{assumption}

\begin{lemma} \label{lem:HardCaseforS}
When $\|s\| \le r $,  algorithm {\ref{algo:full}} returns the global solution of problem ~\ref{eq:cr_subproblem}.
\end{lemma}
\begin{proof}
If  $\|s\| = r $, it is obvious. So the proof will only be given for  $\|s\| < r $.

Because of the way that $\lambda_1$ is chosen, we know that it is a hard case now. Otherwise it cannot be bounded by $r$. So we know $s + \alpha u_1$ is a solution of the first order equation of  problem ~\ref{eq:cr_subproblem}, where $u_1$ is the eignvector of the leftmost eignvalue of $H+\lambda_1$. Thus we choose $a$ so that  $\|s +a u_1\| = r$, and $a$ gives the lower value of equivalent TR problem.

\end{proof}

\begin{lemma} \label{lem:NMforS}
When $\|s\| > r $,  algorithm {\ref{algo:full}} returns the global solution of problem ~\ref{eq:cr_subproblem}.
\end{lemma}
\begin{proof} Since $\| s\| > r$, thus $\phi_1 < 0$. Therefore new $\lambda_1 > -\lambda_{min}$.

Thus, the Newton method for the solution of $ \phi (\lambda)=0$ implemented is well defined.

Thus,algorithm {\ref{algo:full}} converges (See~\cite{ARCP1}).

\end{proof}
\end{comment}

\begin{assumption} \label{as:flowerbound}
The function $f(x)$ is bounded below.
\end{assumption}

\begin{assumption} \label{as:gLipschitz}
$g(x)$ are L-Lipschitz continuous for all $x$.
\end{assumption}

The theorem given below ensures Algorithm {\ref{algo:full}} will solve problem ~\ref{eq:cr_subproblem}, and it can be found in ~\cite{ARCP1} and ~\cite{CoGoTo00b}.
\begin{theorem} \label {thm:CRCONV}
 Algorithm {\ref{algo:full}} returns the global solution of problem ~\ref{eq:cr_subproblem}.
\end{theorem}
\josh{ We are saying that algorithm {\ref{algo:full}} solves the subproblem.  You mean \ref{algo:subproblem} correct?}
 \begin{lemma} \label{lem:xbound}
Suppose that $x_k$ is generated by Algorithm~\ref{algo:full} and assumption~\ref{as:flowerbound} holds, then sequence $\{ x_k \}$ is bounded.
\end{lemma}
\begin{proof}
This is true because of $f(x_k)$ is monotonically decreased.
\end{proof}
\josh{Lemma \label{lem:BoundB} and Theorem \label{thm:BoundBShift} I don't think are needed for \label{thm:firstOrder}.  These were used
to prove convergence for the nonlinear solver which we don't prove yet, correct?}
The following lemma can be found in ~\cite{JustSample}
\begin{lemma} \label{lem:BoundB}
Suppose that $x_k$ is generated by Algorithm~\ref{algo:full} and assumption~\ref{as:gLipschitz} holds, and also $B_k$ is the Hessian
approximations updated by Equation~\ref{eq:SR1update} when the new curvature pair satisfies Equation~\ref{eq:curvature}, then there exists a constant $c_1 > 0$ such that $ \| B_k \| \le c_1$.  
\end{lemma}



Using Lemma~\ref{lem:BoundB}, the following important theorem can be derived, which indicates that the solution $s_k^\ast$ of the cubic regularized subproblem is bounded. 
\josh{ I am not sure this theorem is true without stronger assumptions given Theorem~\ref{thm:gammaeffect}.
We say nothing how we choose $\gamma.$  We can choose $\gamma_k$ if we wanted such that eigenvalues diverge in both directions regardless
of what the algorithm is doing. So maybe we need to state the gamma theorem first, and then state assumptions that prove boundedness?
}

\begin{theorem} \label{thm:BoundBShift}
Suppose that $x_k$ is generated by Algorithm~\ref{algo:full} and assumption~\ref{as:gLipschitz} holds, and also $B_k$ is the Hessian
approximations generated by Equation~\ref{eq:SR1update} when the new curvature pair satisfies Equation~\ref{eq:curvature}, then there exists a constant $c_2 > 0 $ such that $ \| B_k + \sigma_k \|s_k\| I \| \le c_2$  
\end{theorem}
\begin{proof}
\josh{ Could we switch to $B_k = U \Lambda U^T$? sorry I did this in the earlier section.}
We will first show that $\sigma_k \|s_k\|$ is always bounded for all $k$.
\newline Let $B_k = U^T \Sigma U$, and where $\Sigma$ is a diagonal matrix and $U^T U = I $, 

Then, we have:
$B_k + \sigma_k \|x_k\| I = U^T (\Sigma + \sigma_k \|s_k\| I)U$. Therefore,

$(B_k + \sigma_k \|s_k\| I) (B_k + \sigma_k \|s_k\| I) = U^T (\Sigma + \sigma_k \|s_k\| I) (\Sigma + \sigma_k \|s_k\| I) U$

Because of Lemma~\ref{lem:BoundB}, there exists $\lambda_{min}$ and $\lambda_{max}$ such that 
\begin{eqnarray} \label{eq:eignineq01} 
(\sigma_k \|s_k\| + \lambda_{min})^2  & \le & \dfrac{x^T (B_k + \sigma_k \|s_k\| I)(B_k + \sigma_k \|s_k\| I) x }{ x^T x}   \le (\sigma_k \|s_k\| + \lambda_{max})^2 
\end{eqnarray}
, for all $x$.
\newline Set $x = s_{k+1}$ in Equation~\ref{eq:eignineq01}, and because of $s_{k+1}$ is solution of problem ~\ref{eq:cr_subproblem}, we have: 
\begin{eqnarray} \label{eq:eignineq02}
(\sigma_k \|s_k\| + \lambda_{min})^2  & \le & \dfrac{ g_k^T g_k }{ s_{k+1}^T s_{k+1}}   \le (\sigma_k \|s_k\| + \lambda_{max})^2 
\end{eqnarray}
There are two scenarios now.
\begin{enumerate}
    \item $\dfrac{ g_k^T g_k }{ s_{k+1}^T s_{k+1}}$ is bounded. Because of Equation~\ref{eq:eignineq02}, we can easily conclude that $\sigma_k \|s_k\|$ is bounded. Thus, the lemma follows.
    \item $\dfrac{ g_k^T g_k }{ s_{k+1}^T s_{k+1}}$ is unbounded. That is, there exists $M_k \to \infty$ such that $\dfrac{ g_k^T g_k }{ s_{k+1}^T s_{k+1}} \ge M_k$. 
    \newline Because of Lemma~\ref{lem:xbound}, $ g_k^T g_k$ is bounded. We have that $s_k^Ts_k \to 0$ as $\dfrac{ g_k^T g_k }{ s_{k+1}^T s_{k+1}}$ is unbounded.
    Using Taylor expansion, we note that from ~\ref{eq:rho_calc}, 
    \begin{eqnarray*}\label{eq:eignineq03}
\rho_k  &= & \frac{f(x_k) - f(x_k + s_k)}{f(x_k) - m_k(s_k)} \\
&= & \frac{f(x_k) - m_k(s_k) - O(\|s\|^3)}{f(x_k) - m_k(s_k)} \\ 
   \end{eqnarray*}
But as $\|g_k\| \ge M_k \|s_k\|$, we have: 
    \begin{eqnarray*}\label{eq:eignineq04}
{f(x_k) - m_k(s_k)} &= & g_k ^T s_k + s_k^T B_k s_k \\
&\ge & M_k \|s_k\|^2 - c_1 \|s_k\|^2
   \end{eqnarray*}
, when $\|s\|$ is small.
\newline Therefore, when $s_k$ is very small, combining Equation~\ref{eq:eignineq03} and ~\ref{eq:eignineq04}, we have:
    \begin{eqnarray*}\label{eq:eignineq05}
|\rho_k - 1| & = & \frac{O(\|s\|^3)} {f(x_k) - m_k(s_k)} \\
  & \le & \frac{O(\|s\|^3)} {M_k \|s_k\|^2 - c_1 \|s_k\|^2}\\
   \end{eqnarray*}
Because $M_k \to \infty$ We now have that $\rho_k \to 1$ when $\|s_k\| \to 0$. This means that $\sigma_k$ is bounded. 
\newline So, $\dfrac{ g_k^T g_k }{ s_{k+1}^T s_{k+1}}$ is unbounded, we have that $\|s_k\| \to 0$ and $\sigma_k$ is bounded. Therefore $\sigma_k \|s_k\|$ is bounded.
    \end{enumerate}
So, we conclude that $\| B_k + \sigma_k \|s_k\| I \|$ is bounded.  
\end{proof}

We noticed that the leftmost eigenvalue of $B_k$ could become
very negative. When this happens, the following theorem states that the search direction $p_k$ will be independent from $g_k$, but on the eignvectors with respect to the eigenvalues of $B_k$ remaining bounded below. 
\josh{ Theorem  \ref{thm:unboundedeig} and Theorem \ref{thm:delta0} should be proved for fixed $k.$
Theorem \ref{thm:gammaeffect} shows that $B_k(\gamma)$ can have infinite eigenvalues. One theorem shows why this is bad. The other shows that for a fixed
$k$ if we increase $sigma$ we will generate the steepest descent direction.  These are just to prove properties of the step generation, not asymptotic
behavior I think. 
}
\begin {theorem} \label{thm:unboundedeig}
Let $\lambda_1$ be the smallest eigenvalue of $B_k$. Suppose $\lambda_1 \rightarrow -\infty$ as $k \rightarrow \infty,$ and $\sigma_k$ is bounded for all $k$. For Algorithm{\ref{algo:full}}, we then have that the solution of the cubic regularized subproblem, $s_k$ converges to the eigen-space of $B_k$ corresponding to unbounded eigenvalues.
\end{theorem}
\begin{proof}
Let $B_k = W \Lambda_k W^T$ denote the eigen decomposition of $B_k$ where the diagonals
of $\Lambda_k$ satisfy $\lambda_1 \le \lambda_2 \le \cdots \le \lambda_n.$
Let $J$ denotes the maximum integer such that $\lambda_J$ remains bounded. That is, there exists a constant $C$ such that $\lambda_i \ge C$ for all $i \ge J$ as $k \rightarrow \infty.$ 
\newline Then because of  Theorem~\ref{thm:firstorderCR}, we have that the solution of problem~\ref{eq:cr_subproblem} has form
\[
s_k =-\sum_{\lambda_j < C}^n \dfrac{\hat g_k^T w_j}{\lambda_j + \sigma_k \|s_k\|}w_j - 
\sum_{\lambda_j \ge C}^n \dfrac{ \hat g_k ^T w_j}{\lambda_j +  \sigma_k \|s_k\|}w_j,
\]
where $\sigma_k \|s_k\| \ge -\lambda_1$ denotes the smallest eigenvalue of $B_k$. Because $\lambda_1\to -\infty$ we must have that $\sigma_k \|s_k\| \to \infty.$
\newline Thus
$
\left \| \sum_{\lambda_j \ge C}^n \tfrac{\hat g_k^T w_j}{\lambda_j + \sigma_k \|s_k\|}w_j
\right \| \to 0.
$ 
because of Lemma~\ref{lem:xbound}, $g_k$ is bounded. So $s_k$ converges to the space of $\{w_j\}_{\lambda_J < C}$.
\end{proof}
When $B_k$ is very bad approximation of the Hessian. The above theorem indicates that the search direction $p_k$ can be very poor direction to minimize $f(x)$. It is believed that restarting SR1 update can be a good strategy when this happens. 

The following theorem shows that if $\gamma$ is chosen carefully, then the leftmost eigenvalue of$B_k$ going to $-\infty$ can be prevented.
\begin {theorem} ~\cite{erway2020trust}\label{thm:gammaeffect}
Suppose $B_0 = \gamma I$ and that $\hat \lambda$ denotes the smallest eigenvalue of the generalized eigenvalue problem defined below, where $D_k, L_k, S_k$ used are defined in ~\cite{erway2020trust}.
\begin{eqnarray} 
(D_k+L_k+L_k^T)u = \hat \lambda S_k^T S_k u
\end{eqnarray}
Further assume that $\Psi_k$ also defined in ~\cite{erway2020trust}, and $S_k$ are full rank. Then if $\hat \lambda > 0$, we have the following properties:
\begin{enumerate}
    \item $B_k$ is positive definite if $0 < \gamma < \hat \lambda$
    \item As $\gamma \to \hat \lambda $  from below, $\lambda_{max}(B_k) \to \infty$ and $\rm{cond}(B_k)\to \infty$.
    \item As $\gamma \to \hat \lambda$  from above, $\lambda_{min}(Bk) \to -\infty$.
\end{enumerate}
\end{theorem}

The theorem below shows that when $\sigma_k $ is very large, Algorithm~\ref{algo:full} will generate a  direction similar to classical SGD direction.
\begin{theorem} \label{thm:delta0}
When $\sigma_k \to \infty$, direction $s_k$ generated by Algorithm~\ref{algo:full} will converge
to a multiple of $g_k$.
\end{theorem}

\begin{proof}
we first note that
\begin{eqnarray} \label{eq:delta001}
    m_k(s_k) &=& \f(x_k) + s_k^Tg_k + s_k^T( \frac{1}{2} B_k + \frac{1}{3} \sigma_k \|s_k\| I) s_k 
   \end{eqnarray}
Because of Lemma~\ref{lem:BoundB} and Theorem~\ref{thm:BoundBShift}, $\|\frac{1}{2} B_k + \frac{1}{3} \sigma_k \|s_k\| I\|$ is bounded.
\newline It is also easy to see that $\|s_k\| \to 0$ when $\sigma_k \to \infty$ as we are minimizing problem~\ref{eq:cr_subproblem}.

Therefore, when $\|s_k\| \to 0$, $m_k(s_k)$ is dominated by $s_k^Tg_k$ because of Equation~\ref{eq:delta001}.
Thus, direction $s_k$ generated by Algorithm~\ref{algo:full} will converge
to a multiple of $g_k$. 
\end{proof}

\begin{comment}
\begin{theorem} \label{thm:firstOrder}
Suppose that $x_k$ is generated by Algorithm~\ref{algo:full} and assumptions~\ref{as:ferror} and ~\ref{as:hbound} hold, then 
with probability one, we have: 
\begin{eqnarray}\label{eq:convergence}
\lim_{k\to\infty} \inf \|\nabla f(w_k)\| = 0.
\end{eqnarray}
\end{theorem}
\begin{proof}
This can be done.
\end{proof}

\end{comment}

